De Sitter vacua -- when are `subleading corrections' really subleading?

We consider various string-loop, warping and curvature corrections that are expected to appear in type IIB moduli stabilisation scenarios. It has recently been argued, in the context of strongly-warped LVS de Sitter vacua, that it is impossible to achieve parametric suppression in all of these corrections simultaneously \cite{Junghans:2022exo}. We investigate corrections in the context of the recently discovered weakly-warped LVS de Sitter vacua, which represent a distinct branch of solutions in type IIB flux compactifications, supported by small conifold flux numbers $MK \lesssim 32$. Warping corrections become less problematic in this regime, and some corrections even help to reach the weakly-warped regime of parameter space. Other corrections continue to be dangerous and would require numerical coefficients to be computed -- and found to be small -- in order not to destroy the consistency of the weakly-warped LVS de Sitter solution.

==> Sections/cs_moduli_metric.tex <==
\section{Complex structure moduli metric}
\label{sec:complexstructuremoduli}

Here we review the computation of $G_{S\bar{S}}$ for the conifold deformation modulus, $S$, using the KS metric, making explicit the appearance of the volume modulus. We follow closely \cite{douglas2007warping}. 

The metric in the complex structure moduli space can be be computed using 

\begin{align}
    G_{\alpha\Bar{\beta}} = \frac{i\int h~\chi_\alpha\wedge\chi_{\Bar{\beta}}}{i\int h~\Omega\wedge\Bar{\Omega}},
    \label{eq:CS_moduli_metric}
\end{align}

\noindent where now, $h = 1 + \frac{e^{-4A_0(y)}}{c(x)}$. This corresponds to the Kahler potential
%
\begin{align}
    \mathcal{K}_{cs} = -\log\left(\frac{i}{l_s^6}\int h~\Omega\wedge\Bar{\Omega}\right).
\end{align}

In our setup, it is assumed that all complex structure moduli are stabilised in the UV, i.e. in the bulk, except for the deformation modulus $S$ that governs the Klebanov-Strassler geometry and lives in the highly-warped region. In particular, this means we can split the Kahler potential into two different contributions
%
\begin{align}
    \mathcal{K}_{cs} &= -\log\left(\frac{i}{l_s^6}\int h~\Omega\wedge\Bar{\Omega} \right) \nn\\
    &= -\log\left(\frac{i}{l_s^6}\int_{bulk} h~\Omega\wedge\Bar{\Omega} + \frac{i}{l_s^6}\int_{conifold} h~\Omega\wedge\Bar{\Omega} \right) \nn\\
    &\approx -\log\left(\frac{i}{l_s^6}\int_{bulk} \Omega\wedge\Bar{\Omega} + \frac{i}{l_s^6}\int_{conifold} h~\Omega\wedge\Bar{\Omega} \right) \nn\\
    &= -\log\left(\frac{i}{l_s^6}\int_{bulk} \Omega\wedge\Bar{\Omega}
    \left(1 + \frac{i\int_{conifold} h~\Omega\wedge\Bar{\Omega}}{i\int_{bulk} \Omega\wedge\Bar{\Omega}} \right)\right) \nn\\
    &= -\log\left(\frac{i}{l_s^6}\int_{bulk} \Omega\wedge\Bar{\Omega}\right)
    - \log\left(1 + \frac{i\int_{conifold} h~\Omega\wedge\Bar{\Omega}}{i\int_{bulk} \Omega\wedge\Bar{\Omega}} \right) \nn\\
    &\approx \mathcal{K}_{cs}^{UV} +  \frac{e^{\mathcal{K}_{cs}^{UV}}}{l_s^6} i\int_{conifold} h~\Omega\wedge\Bar{\Omega}\nn \\
    &= \mathcal{K}_{cs}^{UV} + \mathcal{K}(S,\Bar{S})\,,
\end{align}

\noindent where the first approximation follows from $h\approx 1$ in the bulk and the second assumes the contribution from the bulk is much bigger than the one from the conifold. 
%
\begin{align}
    \mathcal{K}_{cs}^{UV} &= -\log\left(\frac{i}{l_s^6}\int_{bulk} \Omega\wedge\Bar{\Omega}\right) 
    = -\log\left(\frac{||\Omega||^2V_{6}}{l_s^6}\right)\,.
\end{align}

\iffalse
In \cite{upliftingrunaways2019}, this term is $K_0 = -\log(||\Omega||^2V_w)$, with the definition $V_w = \int\sqrt{g_{6^{(0)}}}(e^{-4A_0(y)} + c)$. Hence, this gives the extra factor of $1/c(x)$ in the potential, when we take the same limit $c(x)\gg e^{-4A_0(y)}$. Implicitly inside the log there is a factor of $1/\alpha'^3$, which makes the argument dimensionless. In fact, if we take the fiducial volume $V_{CY} = \alpha'^3$, we get $K_{cs}^{UV} = -\log ||\Omega||^2$. 
\fi

We can now compute the conifold contribution to the metric following the computations in \cite{douglas2007warping}
%6
\begin{align}
    G_{S\Bar{S}} = \frac{e^{\mathcal{K}_{cs}^{UV}}}{l_s^6}i\int_{conifold} h~\chi_S\wedge\chi_{\Bar{S}}.
\end{align}
%
For the KS metric, the (2,1)-form $\chi_S$ is given by
%
\begin{align}
    \chi_S = g^3\wedge g^4\wedge g^5 + d[F(\eta)(g^1\wedge g^3 + g^2\wedge g^4 )] - id[f(\eta)(g^1\wedge g^2) + k(\tau)(g^3\wedge g^4)],
\end{align}
%
where the functions $f,k,F$ were computed in \cite{KS2000supergravity} 
%
\begin{align}
    F(\eta) = \frac{\sinh{\eta}-\eta}{2\sinh{\eta}} ,
    && f(\eta) = \frac{\eta\coth{\eta}-1}{2\sinh{\eta}}(\cosh{\eta}-1) ,
    && k(\eta) = \frac{\eta\coth{\eta}-1}{2\sinh{\eta}}(\cosh{\eta}+1).
    \label{eq:ansatz_functions_KS}
\end{align}
%
It will be useful to look at the limits $\eta\rightarrow 0$ and $\eta\rightarrow\infty$ of these functions:
%
\begin{align}
    &F(\eta\rightarrow 0) = \frac{\eta^2}{12}\,,
    && f(\eta\rightarrow 0) = \frac{\eta^3}{12}\,,
    && k(\eta\rightarrow 0) = \frac{\eta}{3}\,, \\
    &F(\eta\rightarrow\infty) = \frac{1}{2} -\eta e^{-\eta}\,,
    && f(\eta\rightarrow\infty) = \frac{\eta}{2}\,,
    && k(\eta\rightarrow\infty) = \frac{\eta}{2}\,,
\end{align}
%
Surprisingly the combination we need, $\chi_S\wedge\chi_{\Bar{S}}$, is a total $\eta$-derivative
%
\begin{align}
    \chi_S\wedge\chi_{\Bar{S}} = -\frac{2i}{64\pi^4}d\eta \wedge \left(\prod_i g^i\right) \frac{d}{d\eta}[f+F(k-f)],
\end{align}
%
from which we find for $G_{S\Bar{S}}$ (with all the integrals over the conifold region)
%
\begin{align}
    G_{S\Bar{S}} &= \frac{e^{\mathcal{K}_{cs}^{UV}}}{l_s^6}i\int h~\chi_S\wedge\chi_{\Bar{S}} \nn\\
    &= \frac{i}{||\Omega||^2V_{6}} \int h~\chi_S\wedge\chi_{\Bar{S}} \nn\\
    &= \frac{1}{||\Omega||^2V_{6}} \frac{2}{64\pi^4} \int h~ d\eta \wedge \left(\prod_i g^i\right) \frac{d}{d\eta}[f+F(k-f)] \nn\\
    &= \frac{2}{64\pi^4||\Omega||^2V_{6}} 
    \left(\int \prod_i g^i\right)
    \int d\eta ~h~ \frac{d}{d\eta}[f+F(k-f)] \nn\\
    &= \frac{2}{\pi||\Omega||^2V_{6}}
    \left(\int d\eta \frac{d}{d\eta}\{h~[f+F(k-f)]\}
    - \int d\eta \frac{dh}{d\eta}[f+F(k-f)]
    \right) ,
\end{align}

\noindent where we preformed the $\eta$ integral by parts and used $\int \prod_i g^i = 64\pi^3$. 

We are left with an integral in $\eta$, which corresponds to the radial coordinate of the conifold. We introduce a cutoff scale where the conifold connects to the bulk. For the coordinate defined in the limit $\eta\rightarrow\infty$,
%
\begin{align}
    r_\infty^2 = \frac{3}{2^{5/3}}s^{2/3}e^{2\eta/3},
\end{align}
%
the cutoff scale $\Lambda_{UV}$ is defined as
%
\begin{align}
    \Lambda_{UV}^2 \equiv r_{UV}^2 =  \frac{3}{2^{5/3}}s^{2/3}e^{2\eta_{\Lambda}/3} 
    \implies \eta_\Lambda = \frac{3}{2}\log\frac{2^{5/3}}{3} + \log\frac{\Lambda_{UV}^3}{s}\,,
    \label{eq:Lambda0_def}
\end{align}

\noindent where $\eta_\Lambda$ is the maximum value of $\eta$, i.e. the upper bound of our integral where the conifold connects with the bulk. We see that the first term in the integral is just a boundary term, so it suffices to evaluate $h~[f+F(k-f)]$ at $\eta\rightarrow 0$ and $\eta\rightarrow\eta_\Lambda$ (where we can think of $\eta_\Lambda \gg 1$ and use the approximations for $\eta\rightarrow\infty$). It is useful to recall the warp factor for the deformed conifold, now written in terms of the complex structure $s=|S|=\epsilon^2$
%
\begin{align}
    e^{-4A_0(y)} = 2^{2/3}\frac{(\alpha'g_sM)^2}{s^{4/3}}I(\eta),
    &&
    I(\eta)\equiv \int_{\eta}^{\infty} dx ~ \frac{x\coth(x) - 1}{\sinh^2{x}}(\sinh(2x)-2x)^{1/3}\,,
\end{align}

\noindent At $\eta\rightarrow 0$, $I(0)\approx 0.718$ and $f+F(k-f)=0$, and at $\eta\rightarrow\eta_\Lambda$, in the bulk, $h\approx 1$ and
%
\begin{align}
    f+F(k-f) \approx \frac{\eta_\Lambda}{2} =  \frac{3}{4}\log\frac{2^{5/3}}{3} + \frac{1}{2}\log\frac{\Lambda_{UV}^3}{s}.
\end{align}
%
As for the second term, all we need is the derivative of $h$ 

\begin{align}
    \frac{dh}{d\eta}
    =\frac{1}{c(x)}\frac{de^{-4A_0(y)}}{d\eta} 
    &= 2^{2/3}\frac{(\alpha'g_sM)^2}{s^{4/3}} \frac{1}{c(x)}\frac{dI(\eta)}{d\eta}\nn\\
    &= -4\times 2^{2/3}\frac{(\alpha'g_sM)^2}{s^{4/3}} \frac{1}{c(x)}\frac{f+F(k-f)}{(\sinh(2\eta)-2\eta)^{2/3}}\,,
\end{align}

\noindent and so the second integral (which is well approximated by taking $\eta_\Lambda\to\infty$) gives

\begin{align}
    -4\times  2^{2/3}\frac{(\alpha'g_sM)^2}{s^{4/3}} \frac{1}{c(x)}\int_0^{\eta_\Lambda} \frac{[f+F(f-k)]^2}{(\sinh(2\eta)-2\eta)^{2/3}} 
    \approx 0.093\times  (-4\times 2^{2/3})\frac{(\alpha'g_sM)^2}{s^{4/3}} \frac{1}{c(x)}.
    \label{eq:integral_metric_GSS}
\end{align}

Hence, the metric becomes

\begin{align}
    G_{S\Bar{S}} 
    &= \frac{1}{\pi||\Omega||^2V_{6}} 
    \left(\frac{3}{2}\log\frac{2^{5/3}}{3} + \log\frac{\Lambda_{UV}^3}{s}
    + 0.093\times 8 \times 2^{2/3}\times \frac{(\alpha'g_sM)^2}{s^{4/3}}\frac{1}{c(x)}
    \right) \,.
\end{align}
%
Defining the constant $c' \approx 0.093\times 8 \times 2^{2/3} \approx 1.18$ and for $s\ll\Lambda_{UV}^3$ (which is equivalent to the assumption $\eta_\Lambda\gg 1$), we can neglect the first term 
\begin{align}
    G_{S\Bar{S}}
    = \frac{1}{\pi||\Omega||^2V_{6}} 
    \left(\log\frac{\Lambda_{UV}^3}{s}
    + c' \frac{(\alpha'g_sM)^2}{s^{4/3}}\frac{1}{c(x)}
    \right).
    \label{eq:appendixC_GSS}
\end{align}
%
This metric corresponds to the K\"ahler potential
%
\begin{align}
   \mathcal{K}(S,\Bar{S}) =\frac{1}{\pi||\Omega||^2V_{6}} \left(|S|^2\left(\log\frac{\Lambda_{UV}^3}{|S|} + 1\right) + \frac{9c'(\alpha'g_sM)^2}{c(x)}|S|^{2/3}\right).
\end{align}

We can now make a field redefinition, introducing a dimensionless deformation modulus $z=S/l_s^3$ and identifying the volume modulus $c(x)=\V^{2/3}$
%
\begin{align}
    \mathcal{K}(z,\Bar{z}) =\frac{l_s^6
    }{\pi||\Omega||^2V_{6}}\left(|z|^2\left(\log\frac{\Lambda_0^3}{|z|} + 1\right) + \frac{9c'(g_sM)^2}{(2\pi)^4\V^{2/3}}|z|^{2/3}\right),
\end{align}
where now $\Lambda_0=\Lambda_{UV}/l_s$ is expressed in string units of $l_s$. With this redefinition we can say that ``$z$ is small'', i.e. the dimensionless quantity $|S|/l_s^3\ll 1$ or $|S|$ is small in string units.

Finally, we can make the choice $V_{6}=l_s^6$. Keeping it allows us to keep track of $V_{6}$ and remember where this factor comes from but, being just a volume integral, we can always choose to normalize it in such a way, since the volume modulus keeps the overall volume dependence. 
